Alternative Restart Strategies for CMA-ES

This paper focuses on the restart strategy of CMA-ES on multi-modal functions. A first alternative strategy proceeds by decreasing the initial step-size of the mutation while doubling the population size at each restart. A second strategy adaptively allocates the computational budget among the restart settings in the BIPOP scheme. Both restart strategies are validated on the BBOB benchmark; their generality is also demonstrated on an independent real-world problem suite related to spacecraft trajectory optimization.

==> ppdata/ppfigs.tex <==
% Do not modify this file: calls to post-processing software will overwrite any modification.
Legend: {\color{blue}$\circ$}: BIPOP-aCMA, {\color{red}$\triangledown$}: IPOP-aCMA, {\color{cyan}$\star$}: NBIPOP-aCMA, {\color{magenta}$\Box$}: NIPOP-aCMA

==> ppdata/pprldmany_40D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algaperfprof}{\StrLeft{BIPOP-aCMA}{\nperfprof}}\providecommand{\algbperfprof}{\StrLeft{IPOP-aCMA}{\nperfprof}}\providecommand{\algcperfprof}{\StrLeft{NBIPOP-aCMA}{\nperfprof}}\providecommand{\algdperfprof}{\StrLeft{NIPOP-aCMA}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{\mbox{\algbperfprof}
\vfill \mbox{\algdperfprof}
\vfill \mbox{\algzeroperfprof}
\vfill \mbox{\algcperfprof}
\vfill \mbox{\algaperfprof}}


==> ppdata/pprldmany_40D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algaperfprof}{\StrLeft{BIPOP-aCMA}{\nperfprof}}\providecommand{\algbperfprof}{\StrLeft{IPOP-aCMA}{\nperfprof}}\providecommand{\algcperfprof}{\StrLeft{NBIPOP-aCMA}{\nperfprof}}\providecommand{\algdperfprof}{\StrLeft{NIPOP-aCMA}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{\mbox{\algzeroperfprof}
\vfill \mbox{\algdperfprof}
\vfill \mbox{\algaperfprof}
\vfill \mbox{\algcperfprof}
\vfill \mbox{\algbperfprof}}


==> ppdata/pptables_f001_40D.tex <==
\providecommand{\ntables}{7}\providecommand{\algatables}{\StrLeft{BIPOP-aCMA}{\ntables}}\providecommand{\algbtables}{\StrLeft{IPOP-aCMA}{\ntables}}\providecommand{\algctables}{\StrLeft{NBIPOP-aCMA}{\ntables}}\providecommand{\algdtables}{\StrLeft{NIPOP-aCMA}{\ntables}}
\begin{tabularx}{1.03\textwidth}{@{}c@{}|*{6}{@{}r@{}X@{}}|@{}r@{}@{}l@{}}
$\Delta f_\mathrm{opt}$ & \multicolumn{2}{@{\,}X@{\,}}{1e1} & \multicolumn{2}{@{\,}X@{\,}}{1e0} & \multicolumn{2}{@{\,}X@{\,}}{1e-1} & \multicolumn{2}{@{\,}X@{\,}}{1e-3} & \multicolumn{2}{@{\,}X@{\,}}{1e-5} & \multicolumn{2}{@{\,}X@{}|}{1e-7} & \multicolumn{2}{@{}l@{}}{\#succ}\\\hline
\textbf{f1} & \multicolumn{2}{@{\,}X@{\,}}{83} & \multicolumn{2}{@{\,}X@{\,}}{83} & \multicolumn{2}{@{\,}X@{\,}}{83} & \multicolumn{2}{@{\,}X@{\,}}{83} & \multicolumn{2}{@{\,}X@{\,}}{83} & \multicolumn{2}{@{\,}X@{\,}|}{83} & 15 & /15\\
\algatables\hspace*{\fill} & 9 & .4 & 15 &  & 21 &  & 33 &  & 45 &  & 58 &  & 15 & /15\\
\algbtables\hspace*{\fill} & \textbf{9} & \textbf{.3} & \textbf{15} & \textbf{} & \textbf{21} & \textbf{} & \textbf{33} & \textbf{} & \textbf{45} & \textbf{} & \textbf{57} & \textbf{} & 8 & /8\\
\algctables\hspace*{\fill} & 9 & .5 & 15 &  & 22 &  & 34 &  & 46 &  & 58 &  & 15 & /15\\
\algdtables\hspace*{\fill} & 10 &  & 15 &  & 21 &  & 34 &  & 46 &  & 58 &  & 15 & /15
\end{tabularx}

==> ppdata/pptables_f002_40D.tex <==
\providecommand{\ntables}{7}\providecommand{\algatables}{\StrLeft{BIPOP-aCMA}{\ntables}}\providecommand{\algbtables}{\StrLeft{IPOP-aCMA}{\ntables}}\providecommand{\algctables}{\StrLeft{NBIPOP-aCMA}{\ntables}}\providecommand{\algdtables}{\StrLeft{NIPOP-aCMA}{\ntables}}
\begin{tabularx}{1.03\textwidth}{@{}c@{}|*{6}{@{}r@{}X@{}}|@{}r@{}@{}l@{}}
$\Delta f_\mathrm{opt}$ & \multicolumn{2}{@{\,}X@{\,}}{1e1} & \multicolumn{2}{@{\,}X@{\,}}{1e0} & \multicolumn{2}{@{\,}X@{\,}}{1e-1} & \multicolumn{2}{@{\,}X@{\,}}{1e-3} & \multicolumn{2}{@{\,}X@{\,}}{1e-5} & \multicolumn{2}{@{\,}X@{}|}{1e-7} & \multicolumn{2}{@{}l@{}}{\#succ}\\\hline
\textbf{f2} & \multicolumn{2}{@{\,}X@{\,}}{796} & \multicolumn{2}{@{\,}X@{\,}}{797} & \multicolumn{2}{@{\,}X@{\,}}{799} & \multicolumn{2}{@{\,}X@{\,}}{800} & \multicolumn{2}{@{\,}X@{\,}}{802} & \multicolumn{2}{@{\,}X@{\,}|}{804} & 15 & /15\\
\algatables\hspace*{\fill} & 38 &  & 45 &  & 49 &  & 55 &  & 57 &  & 59 &  & 15 & /15\\
\algbtables\hspace*{\fill} & 37 &  & \textbf{43} & \textbf{} & 48 &  & 55 &  & 57 &  & \textbf{58} & \textbf{} & 8 & /8\\
\algctables\hspace*{\fill} & 37 &  & 43 &  & \textbf{47} & \textbf{} & \textbf{53} & \textbf{} & 57 &  & 59 &  & 15 & /15\\
\algdtables\hspace*{\fill} & \textbf{37} & \textbf{} & 43 &  & 48 &  & 53 &  & \textbf{57} & \textbf{} & 58 &  & 15 & /15
\end{tabularx}
